Thermal Spectra of Warped and Broken Accretion Disks

Black holes may accrete gas with angular momentum vectors misaligned with the black hole spin axis. The resulting accretion disks are subject to Lense-Thirring precession, and hence torque. Analytical calculations and simulations show that Lense-Thirring precession will warp, and, for large misalignments, fracture the disk. In GRMHD simulations, the warping or breaking occurs at $\lesssim10r_s$, where $r_s$ is the Schwarzschild radius. Considering that accretion disk spectra in the soft state of stellar-mass black holes are generally well modeled as multicolor blackbodies, the question arises as to how consistent warped and broken disks are with observations. Here, we analytically calculate thermal spectra of warped and broken disks with a warp or break radius at $10r_s$ for various disk inclinations. Due to self-irradiation and the projected area of the inclined disk regions, the spectra of inclined disks significantly deviate from multicolor blackbodies and do not follow the multicolor blackbody relation $\nu L_\nu\propto\nu^{\gamma}=\nu^{4/3}$ at low frequencies $\nu$. The power-law indices at low frequencies of the inclined disks vary with viewing angle; when viewed face-on, they vary between $\gamma\approx0.91-1.26$ for the warped disks and $\gamma\approx1.37-1.54$ for the broken disks depending on the inclination angle. The differences decrease when moving the location of the disk warp and break to larger radii; for inclined disks to emit as multicolor blackbodies, they must warp or break at radii $\geq50r_s$. Our results imply that accretion disks around black holes in the soft state warp or break at larger radii than suggested in GRHMD simulations.

==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
%Misalignment between the black hole spin and the angular momentum vector of the accretion flow induces Lense-Thirring precession precession, which has been suggested to cause observed jet precessions and has been inferred 

Misalignments between the black hole spin axis and the angular momentum vector of the accretion flow have been suggested observationally by precessing jets and gravitational wave measurements \citep[e.g,][]{Hjellming1995Natur.375..464H,OShaughnessy2017PhRvL.119a1101O,Cui2023Natur.621..711C}. In simulations, the induced Lense-Thirring precession
warps or breaks the disk depending on the inclination angle. Recent GRMHD simulations of tilted disks showed that disk warping or breaking occurs at $r\lesssim10r_s$ %\jsp{$\lesssim20r_g$} 
\citep[e.g.,][]{Liska2019MNRAS.487..550L,Liska2021MNRAS.507..983L,Liska2022ApJS..263...26L}, while smoothed particle hydrodynamic simulations and analytical calculations place the radius of disk warping or breaking at larger radii \citep[e.g.,][]{Kumar1985MNRAS.213..435K,Nixon2012ApJ...757L..24N}. In this paper, we analytically calculated the thermal emission of warped and broken disks for a variety of disk inclinations and viewing angles (section \ref{sec:methods}), using a similar warp or break radius $\rbent$ as in GRMHD simulations. We find significant differences between inclined and flat disk spectra due to self-irradiation and the projected area of the inclined disk regions (section \ref{sec:results}). The differences are expected to increase when considering a more physical accretion disk setup with e.g., density variations, and should be observable in the X-ray band (section \ref{sec:discussion}). The inclined disk spectra converge towards the multicolor blackbody solution with increasing $\rbent$. While the inferred differences between flat and inclined disk spectra will depend on the disk inclination and the energy band observed, our results suggest that $\rbent$ needs to be $\geq50r_s$ to agree with observations of stellar-mass black holes in the soft state, which can generally be well described with multicolor blackbody spectra. The alternative interpretation is that disk warping or breaking is not common for black hole systems. However, that argument would not be able to reconcile the jet precession observed for the stellar-mass black hole system GRO J1655-40 \citep[][]{Hjellming1995Natur.375..464H}, whose disk emission can be well described as originating from a flat disk \citep[e.g.,][]{Zhang1997ApJ...479..381Z,Sobczak1999ApJ...520..776S,Shafee2006ApJ...636L.113S}.%\citep[e.g.,][]{Kallman2009ApJ...701..865K,Reis2009MNRAS.395.1257R}. %\jsp{This is new: Moreover, our results align with the observations of MAXI J1820 + 070 \citep[][]{Thomas2022MNRAS.509.1062T}. The black hole system underwent an outburst in 2018}
% \ob{These references look at warm absorber and reflection spectra, respectively.  It would be better to cite some continuum spectral fittings that show more directly that the soft state disks can be fitted by a standard flat disk multi-temperature (color-corrected) blackbody.}

%\jsp{to do: mention  GRO J1655 - 40}%However, if disk warping would occur as close to the black hole as suggested by GRMHD simulations, the alternative interpretation would be that black holes in the soft state tend to be surrounded by flat or at most very slightly warped disks.

The comparison between inclined and flat disk spectra presented in this paper might hold implications beyond black holes in the soft state. Low-frequency quasi-periodic oscillations (QPOs) are common in the hard and intermediate state \citep[for a review, see e.g.,][]{Motta2016,Ingram2019}. The preferred model for Type C QPOs is Lense-Thirring precession of the inner hot accretion flow \citep{Ingram2009MNRAS.397L.101I}. However, if the inner hot accretion flow is misaligned enough to cause Lense-Thirring precession, the misalignment should be able to persist in the accretion disk in the soft state. For Type C QPOs to occur in the hard and intermediate state and the misaligned soft state accretion disk to radiate as a multicolor blackbody, $\rbent$ has to vary significantly between spectral states. More work is needed to determine the properties setting the location of the disk warp or break, and how the location changes with the spectral state of the black hole. 

% Lense-Thirring precession has been suggested as an origin of quasi-periodic oscillations \citep[QPOs]{Ingram2009MNRAS.397L.101I}, which are most often observed in the hard and intermediate state \citep[for a review, see e.g.,][]{Motta2016,Ingram2019}. In the suggested model, QPOs arise through the precession of the inner hot accretion flow. If QPOs can form for accretion flows emitting like multicolor blackbodies in the soft state, then the accretion flow structure must fundamentally change, allowing $\rbent$ to move to significantly smaller radii, or the precession arises due to factors other than an angular momentum misalignment. More work is needed to determine the properties setting the location of the disk warp or break, and how the location changes with the spectral state of the black hole. \ob{I think we need to say something more like LT precession is a favorable model for (Type C) LFQPOs, and requires a source of misalignment.  But then this has implications if the soft state disk is also misaligned.  Then conclude with your "more Work is needed" sentenc.}




% While analytical calculations and smoothed particle hydrodynamic simulations cannot capture all physical processes

==> discussion.tex <==
\section{Discussion}\label{sec:discussion}
The calculations of the spectra of inclined disks %spectra
presented in section \ref{sec:results} are based on simplified accretion disk models (section \ref{sec:methods}). In this section, we discuss the impact of complexities present in physical inclined disks.

We assumed the inclined disks to be infinitely thin, but physical accretion disks extend vertically due to pressure support \citep[e.g.,][]{Blaes2006ApJ...645.1402B,Gu2012ApJ...753..118G}. Self-irradiation will heat the disk and inflate it further, which increases the projected area of the outer disk regions for observers viewing the disk at close to edge-on, and for inner disk regions irradiating them. Accounting for the disk height will therefore enhance the low-energy emission observed at viewing angles close to $\pi/2$, and move the outer disk spectral contribution to higher energies due to increased heating. 

% Hence the disk thickness could increase $Q_{irr}$ (eq.\ref{eq:qint}) and thus the spectral impact of the disk inclination, which will especially be visible at large $\mu$.

A physical accretion disk may also not radiate everywhere as a blackbody. Blackbody emission requires an optically thick accretion disk, but the density of simulated warped and broken disks varies \citep[e.g.,][]{Nealon2015MNRAS.448.1526N,Liska2019MNRAS.487..550L,Liska2021MNRAS.507..983L}, leading to optical depth variations \citep[e.g.,][]{Liska2023ApJ...944L..48L}. Optically thin regions would emit nonthermal radiation, increasing the deviations from a multicolor blackbody further. %\ob{I am not sure what this means.  Energy balance will still cause these regions to emit the same amount of accretion power, but with a strong, hard color correction, i.e. a strong deviation from a blackbody at the same effective temperature.}
The thinning of the inclined disk regions could thus not compensate for their geometrical impact. %For broken disks, density variations could only eliminate the geometrical impact of the inclined regions if the variations led to the innermost flat disk region being cleared out. However, 
Density variations are therefore not expected to eradiacate the differences between warped or broken and flat disk spectra.
%would therefore expectantly the reduce the impact of self-irradiated heating on the disk spectrum, but are unlikely to eradicate the deviations from flat disk spectra.

Accretion disk dynamics present in inclined disks might also alter their spectra. In broken disks, the interaction between gas in the inclined and the flat plane could cause shocks \citep{Kaaz2023ApJ...955...72K}. The shocked gas will radiate at higher energies and with a spectral distribution following a powerlaw \citep[e.g.,][]{Blandford1978ApJ...221L..29B}. Besides the spectral impact of the powerlaw shape, the shocked gas in the inner disk region also increases the irradiation the outer disk regions. Additional shock heating is thus expected to affect the shape of the inclined disk spectra at high energies, due to the modified distribution of the inner disk emission, and enhance %pronounce
the spectral impact of the outer region, due to their stronger irradiation. 

The energy band of the disk spectrum, and thus the band where the power-law index agrees with the multicolor blackbody solution, will furthermore depend on the mass of the black hole and its accretion rate. Decreasing $\dot{M}$ decreases $Q_v$ and $Q_{irr}$, moving the disk spectrum to lower energies. Note that because both heating rates depend on $\dot{M}$, self-irradiation will remain important for large radii of warped disks. The spectrum will also shift to lower energies with increasing black hole mass. However, the spectral shift due to varying $\dot{M}$ and $M$ is minor; the disk temperature due to viscous heating (eq. \ref{eq:qv}) decreases as $\dot{M}^{1/4}$ and $M^{-1/4}$. Therefore, reducing $\dot{M}$ to $0.02\dot{M}_{Edd}$ would still lead to $\gamma\approx4/3$ in the $0.2-0.5$ keV range for a flat disk but to $\gamma$ varying between $0.2-0.96$ for $\mu$ between $0$ and $0.5\pi$ for a warped disk with $\thmax=0.3\pi$. Moving the low-energy disk emission with $\gamma=4/3$ out of the X-ray band would thus require a significant reduction in $\dot{M}$, disagreeing with the Eddington ratios inferred for the soft state of black holes \citep[e.g.,][]{Maccarone2003A&A...409..697M}. Likewise, a significant increase in black hole mass would be necessary to remove the emission less energetic than at the spectral peak from the X-ray band. However, this black hole mass increase would disqualify the black hole from the stellar-mass category \citep[e.g.,][]{Corral2016A&A...587A..61C}, which has been the focus of this study. Hence, for stellar-mass black holes accreting through a misaligned accretion disk with $\rbent=10r_s$ and $\dot{M}\geq0.02\dot{M}_{Edd}$, the discrepancy from a multicolor blackbody should be noticeable.

%The emission of the inner disk region more strongly deviating from a multicolor blackbody and it i, increases in gas temperature are unlikely to diminish the differences of inclined disks emission to a multicolor blackbody emission.



% \begin{itemize}
%     \item assumed that the disk is very thin
%     \begin{itemize}
%         \item disk heating will inflate disk
%         \item could projected area of outer region
%     \end{itemize} 
%     \item warp radius could be somewhere else
%     \item shock heating in broken disk simulations
%     \item assumed that disk is optically thick everywhere
%     \item did not include the irradiated disk irradiating back   
%     \begin{itemize}
%         \item will increase inner disk region temperature
%         \item need heating/cooling function to find equilibrium/ final temperature (beyond the scope of this paper)
%     \end{itemize}
% \end{itemize}


==> emission.tex <==
\subsection{Disk temperature}\label{subsec:diskTemperature}
% \jsp{I have replaced $r_\mathrm{in}$ with $r_\mathrm{isco}$ in eq. \ref{eq:qv} and \ref{eq:ldisktheory}, and wrote at the beginning that this applies for the disk extending to $r_\mathrm{isco}$.}

% The disk temperature is set by viscous heating and by self-irradiation. 
For a standard accretion disk extending down to the $r_{\mathrm{isco}}$, the viscous heating rate is \citep{Shakura1973A&A....24..337S}
\begin{equation}
   Q_v =  \frac{3 G M \dot{M}}{8\pi r^3}\anglB{1-\sqrt{\frac{r_\mathrm{isco}}{r}}}.\label{eq:qv}
\end{equation}
We set the mass accretion rate $\dot{M}$ to $0.05\dot{M}_{Edd}$, where $\dot{M}_{Edd}$ is the Eddington mass accretion rate and related to the Eddington luminosity $L_{Edd}$ as $\dot{M}_{Edd} = L_{Edd}/\anglB{0.1 c^2}$. For pure hydrogen accretion, $\dot{M}\approx7\times10^{17}$ gs\textsuperscript{-1}.

In standard accretion disk theory, integrating eq.\ref{eq:qv} over the entire accretion disk gives the disk luminosity
\begin{equation}
    L_{d} = \int_0^{2\pi}\int_{r_\mathrm{isco}}^\infty Q_v \,dA = \frac{GM\dot{M}}{2r_\mathrm{isco}}, \label{eq:ldisktheory}
\end{equation}
and is $\approx1.6\times10^{38}$ erg s\textsuperscript{-1} for our setup. Evaluating eq.\ref{eq:ldisktheory} between $r_\mathrm{isco}$ and $\rout$ for our inclined disks yields deviation from the theoretical value of $\lesssim0.2\%$, proving that $\rout$ is sufficiently large (the spatial integration is described in section \ref{subsec:numericalEvaluation})

% We start the integration at $r = \anglB{1+10^{-5}}r_s$ instead of $r_{\mathrm{in}}=r_s$ to avoid $Q_v$ (eq.\ref{eq:qv}) becoming zero. 

\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{figures/irradiationSetup.png}
    \includegraphics[width=0.45\linewidth]{figures/visibilityExplained2.png}
    \vspace{-15mm}
    \caption{Left panel: Irradiation of $P(r,\phi)$ by disk element $dA$ \citep[see also][]{Fukue1992PASJ...44..663F}. The point $P(r,\phi)$ and $dA$ are a distance $R$ (grey dot-dashed line) apart. The unit vector $\vprint{d}$ (blue vector) points from $P(r,\phi)$ to $dA$. The normal vectors at $P(r,\phi)$ and $dA$ are $\vprint{n}_P$ (green dashed vector) and $\vprint{n}_i$ (red striped vector) respectively. Right panel: Illustration of the visibility between points on the upper warped disk surface. Points on the concave part on the disk (points A, blue star, and B, orange dot) can irradiate each other. Points on the convex part (points C, cyan cross, and D, pink diamond) can not irradiate each other. A point $P_1\anglB{r,0<\phi_1<\pi}$ (e.g., points A and B) can irradiate another point $P_2\anglB{r,\pi<\phi_2<2\pi}$ (e.g., points C and D) and vice versa if the angle between the line connecting the points and the normal vector at $P_2$ is less than $\pi/2$ (satisfied for B and C, but not for B and D).}%\jsp{I am wondering how helpful the right panel is. I also have another version in the "figures" folder named "visibilityExplained.png" without the lines.} \ob{I THINK I PREFER THE VERSION WITHOUT THE LINES.}}
    \label{fig:irradiationSetup}
\end{figure}

%The inclination of the disk also leads to heating through
%\jsp{I changed $\vprint{l}$ to $\vprint{d}$ to avoid potential confusion with the $\curlB{l_x,l_y,l_z}$ vector.}
A warped or broken disk will irradiate itself \citep[left panel of Fig. \ref{fig:irradiationSetup} for a warped disk; see also][]{Fukue1992PASJ...44..663F}. An infinitesimal disk element $dA$ (eq.\ref{eq:dawr} or \ref{eq:dabr} depending on the disk setup) with a local temperature $T$ irradiates a point $P(r,\phi)$ with an intensity $I = \sigma T^4/\pi$, assuming the disk radiates as a blackbody everywhere. The unit vector \vprint{d} (blue vector) points from $P(r,\phi)$ to $dA$, which is a distance $R$ (grey dot-dashed line) away. The normal vectors at $P(r,\phi)$ and $dA$ are called $\vprint{n}_{\mathrm{P}}$ (green dashed vector) and $\vprint{n}_{\mathrm{i}}$ (red striped vector) respectively. The heating due to irradiation $dQ_{irr}$ of $P(r,\phi)$ due to $dA$ is \citep[see also][]{Fukue1992PASJ...44..663F},
\begin{equation}
    dQ_{irr} = \frac{I}{R^2}\absB{\anglB{-\vprint{d}\cdot\vprint{n}_{\mathrm{i}}}\anglB{\vprint{d}\cdot\vprint{n}_{P}}\anglB{\vprint{n}_{P}\cdot\vprint{n}_{\mathrm{i}}}}\,dA.\label{eq:dQirr}
\end{equation}
Eq. \ref{eq:dQirr} assumes no albedo. While the albedo will be nonzero in the inner disk regions, we are focusing on the impact of the inclined outer regions, where a zero albedo is a reasonable assumption \citep[e.g.,][]{Taverna2020MNRAS.493.4960T}. 
% \ob{It might be worth remarking that you are assuming a zero albedo - i.e. all incident radiation is absorbed rather than reflected.  Is this justified?}  
We also neglect light bending, which would increase the irradiation of the inner disk region and reduce the amount of irradiation at large radii due to the emission from small radii. However, light bending would mostly impact the emission originating close to the black hole, and would therefore not significantly contribute to any deviations from the flat disk solution due to the disk inclination at large radii.

%the effect of light bending decreases with distance and is therefore only significant for the innermost disk regions. 
% We therefore do not expect that the omission of light bending will significantly alter the emission of the inclined disk region.  
%\ob{Because we focus on deviations in the low energy portion of the spectrum that arise from larger radii.}

% We assume that every point of the disk radiates as a blackbody. The total intensity is thus $\sigma T^4/\pi$, with $T$ being the temperature at the irradiating disk element $dA$ and is solved for iteratively. In the first iteration, $T$ is set by viscous heating (eq.\ref{eq:qv}), $T = \anglB{Q_v/2\sigma}^{1/4}$. In the subsequent iterations, we account for heating through self-irradiation and calculate $T$ as $T = \squB{\anglB{Q_v+Q_{irr}}/2\sigma}^{1/4}$.
% integral of the blackbody function $B_\nu$ over frequencies $\nu$
% \begin{equation}
%     I = \int_{\nu_l}^{\nu_h}B_\nu(T)\,d\nu,\label{eq:intensityIntegral}.
% \end{equation}
% We evaluate eq.\ref{eq:bb} for a uniformly spaced 500-entry long frequency grid ranging from $\nu_l = 0.1$keV$/h\approx2.4\times10^{16}$ Hz to $\nu_h=100$ keV$/h\approx2.4\times10^{19}$ Hz via the trapezoidal method.  \ob{Perhaps specify explicitly that $I$ is a function of radius through $T$.  Also, why evaluate the integral numerically when the result is known for $\nu_l=0$ and $\nu_h=\infty$?  Then $I=\sigma T^4/\pi$.}

% The blackbody function is
% \begin{equation}
%     B_\nu(T) = \frac{2h\nu^3/c^2}{\exp\anglB{h\nu/kT}-1}.\label{eq:bb}
% \end{equation}
% The temperature $T$ is set by viscous heating (eq.\ref{eq:qv}) at the irradiating point, $T = \anglB{Q_v/2\sigma}^{1/4}$. 

We integrate $dQ_{irr}$ (eq.\ref{eq:dQirr}) over the entire accretion disk (the spatial integration is described in section \ref{subsec:numericalEvaluation}). Any point $P(r,\phi)$ will only be irradiated by area elements in its line of sight (right panel of Fig. \ref{fig:irradiationSetup}). The top surface of the warped disk between $0<\phi<\pi$ is concave and convex between $\pi<\phi<2\pi$. Two points between $0<\phi<\pi$ (e.g., points A, blue star, and B, orange dot) can thus always irradiate each other and between $\pi<\phi<2\pi$ (e.g., points C, cyan cross, and D, pink diamond) never irradiate each other . A point $P_1\anglB{r_1,0<\phi_1<\pi}$ can irradiate another point $P_2\anglB{r_2,\pi<\phi_2<2\pi}$ and vice versa if the angle between $\overrightarrow{P_1P_2}$ and $\vprint{n}_{P_1}$ is less than $\pi/2$ (Point B and C, but not B and D). The integral of eq.\ref{eq:dQirr} gives the irradiation onto the upper warped disk surface at $P(r,\phi)$. Due to symmetry, evaluating eq.\ref{eq:dQirr} at $P(r,\phi+\pi)$ yields the bottom irradiation at $P(r,\phi)$. 

Two points on the broken disk can irradiate each other if they are not on the same plane. The absolute value of the dot products in eq.\ref{eq:dQirr} accounts for both disk surfaces, so integrating eq.\ref{eq:dQirr} gives the total heating due to irradiation $Q_{irr}$ for the broken disk at $P(r,\tilde{\phi})$. 

The total heating due to irradiation at point $P(r,\phi)$ is thus
\begin{equation}
     Q_{irr}\bigg\rvert_{P( r,\phi)} = \left\{\begin{matrix}
    \int dQ_{irr}\bigg\rvert_{P( r,\phi)}+\int dQ_{irr}\bigg\rvert_{P(r,\phi+\pi)}
 &  \mathrm{warped\,disk}\\
\int dQ_{irr}\bigg\rvert_{P( r,\tilde{\phi})} &  \mathrm{broken\,disk}\\
\end{matrix}\right. .\label{eq:qint}
\end{equation}
Due to the disk symmetries (Fig. \ref{fig:warpedDisk}, \ref{fig:brokenDisk}), $Q_{irr}$ (eq.\ref{eq:qint}) is the same for all quadrants. To sample the whole disk, we calculate $Q_{irr}$ for 24 angles between 0 and $\pi/2$ and for 24 angles between $\pi$ and $3\pi/2$ at different radii.

Self-irradiation heats the disk, increasing the emission intensity. We therefore iterate the $Q_{irr}$ calculations until convergence. The disk temperature is initially set by viscous heating (eq.\ref{eq:qv}), and then by viscous heating and self-irradiation, $T = \squB{\anglB{Q_v+Q_{irr}}/2\sigma}^{1/4}$, in the subsequent iterations. %In the subsequent iterations, we account for self-irradiation and calculate $T$ as $T = \squB{\anglB{Q_v+Q_{irr}}/2\sigma}^{1/4}$. T
The inner disk region is the greatest source of radiation, but its temperatures change negligibly through self-irradiation due to the comparatively low temperatures at larger radii. Heating through self-irradiation therefore converges quickly, and we stop after the third iteration, which changed $Q_{irr}$ by less than $5\%$ for all $\thmax$.

\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/heatingBoth.png}
    \caption{Heating of warped (left panel) and broken (right panel) disks with $\thmax=0.3\pi$. The accretion disks are heated through viscous heating (black lines, eq. \ref{eq:qv}), and self-irradiation (eq. \ref{eq:qint}). We iterated eq. \ref{eq:qint} three times to account for the self-irradiation increasing the irradiating intensity when calculating $Q_{irr}$. Self-irradiation is radially and angle dependent, decreasing with radius and being at a maximum at $\phi=\pi/2$ (red dotted lines) and a minimum at $\phi=0$ (blue dashed line in the left panel, zero for a broken disk and thus not plotted).}%\jsp{both panels are updated}}
    \label{fig:heating}
\end{figure*}
Fig. \ref{fig:heating} shows $Q_v$ (black solid lines, eq.\ref{eq:qv}) and $Q_{irr}$ for $\phi = \pi/2$ and $\phi=0$ (eq.\ref{eq:qint}) for a warped (left panel) and a broken disk (right panel) with $\thmax=0.3\pi$. For the broken disk (right panel), $Q_{irr}$ is measured at $\Tilde{\phi}$. The heating due to self-irradiation reaches a minimum at $\phi=0$ (blue dashed line in the left panel, zero for the broken disk and thus not plotted) and $\phi=\pi$ and a maximum at $\phi=\pi/2$ (red dotted lines) and $\phi=3\pi/2$ for either disk setup.  At small radii, $Q_{irr}$ at $\phi=\pi/2$ are similar for both inclined disks and significantly smaller than $Q_v$. At $2r_s$ for instance, $Q_v$ is $\sim 3800$ times greater than $Q_{irr,\phi=\pi/2}$ of the warped disk and $\sim3200$ times greater than for the broken disk. The hot inner disk region will emit radiation at high energies; we therefore expect $Q_v$ to mostly drive the high-energy emission.

However, $Q_{irr}$ of a warped disk decreases slower with radius than $Q_v$ and therefore becomes increasingly important at larger radii. After an increase of $Q_{irr}$ at $\rbent$ for $\phi=\pi/2$ (left panel in Fig. \ref{fig:heating}, red dotted line), $Q_{irr,\phi=\pi/2}$ surpasses $Q_v$ at $r\approx70r_s$. Since the warped disk is approximately flat at $\phi=0$, $Q_{irr,\phi=0}$ (left panel, blue dashed line) does not increase at $\rbent$. With $Q_{irr}$ dominating over $Q_v$ in the cooler disk regions, self-irradiation is expected to noticeably impact the low-energy emission of warped disks.

% \jsp{Regarding your comment at the end of the result section about self-irradiation, I could add the following here: This impact of self-irradiation will also apply for lower mass accretion rates, because lowering $\dot{M}$ decreases both $Q_{irr}$ and $Q_v$.}
% the disk inclination increases $Q_{irr}$ in the inclined disk regions. The self-irradiated heating of the warped disk at $\phi=\pi/2$ (left panel in Fig. \ref{fig:heating}, red dotted line) increases smoothly at $\rbent$. After $\rbent$, $Q_{irr}$ decreases with radius slower than $Q_v$. , and surpasses $Q_v$ at $r\approx57r_s$. Note that the $Q_{irr}$ increase and subsequent slower decline is not present at $\phi=0$ (left panel, blue dashed line), because the warped disk remains flat at that angle (Fig. \ref{fig:warpedDisk}). With $Q_{irr}$ at $\phi=\pi/2$ dominating in the cooler disk regions, self-irradiated heating of the warped disk is expected to noticeably impact the low-energy emission. 

For broken disks, $Q_{irr}$ at $\Tilde{\phi}=\pi/2$ (right panel in Fig. \ref{fig:heating}, red dotted line) increases abruptly at $\rbent$ due to the disk discontinuity. Beyond $\rbent$, $Q_{irr,\Tilde{\phi}=\pi/2}$ decreases like $Q_v$; fitting a power-law to the heating rates for $r\geq \rbent$ yields a radial dependence of about $r^{-3}$ for both. Since $Q_{irr}$ is always $\gtrsim3$ times smaller than $Q_v$ for a broken disk, self-irradiation will be less important than for warped disks. Nevertheless, the geometrical aspect of the inclined disk region will still impact the spectrum.

%the discontinuity of the broken disk causes $Q_{irr}$ to sharply increase at $\rbent$, while $Q_{irr}$ increases smoothly for the warped disk. At larger radii, $Q_{irr}$ decreases with radius more quickly for the broken than for the warped disk. The warped disk's $Q_{irr}$ at $\phi=\pi/2$ surpasses $Q_v$ at $r\approx57r_s$. However, $Q_{irr}$ is at that radius and angle already about 4 magnitudes smaller than the peak $Q_v$.

\subsection{Disk spectrum}\label{subsec:diskspec}
% \jsp{I still need to mention the energy conservation.}
The accretion disk spectrum as a function of frequency $\nu$ is calculated as 
\begin{equation}
  \nu L_\nu = \frac{2h\nu^4}{c^2}
  \int \frac{\absB{cos \beta}\,dA}{f_{c}^4\squB{\exp\anglB{h\nu/kf_cT}-1}},  \label{eq:nuFnu}
\end{equation}

 % \begin{equation}
%     B_\nu(T) = \frac{2h\nu^3/c^2}{\exp\anglB{h\nu/kT}-1}.\label{eq:bb}
% \end{equation}
where $k$ is the Boltzmann constant and $h$ the Planck constant. We interpolate $Q_{irr}$ (eq.\ref{eq:qint}) with radii and angles to obtain disk temperatures for every angular and radial increment of the spatial integral (section \ref{subsec:numericalEvaluation}).
%The temperature $T = \squB{\anglB{Q_v+Q_{irr}}/2\sigma}^{1/4}$ is set by the total heating rate $Q_{tot}=Q_v+Q_{irr}$ (eq. \ref{eq:qv}, \ref{eq:qint}). 
 

The color correction factor $f_c$ is \citep[][]{Done2012MNRAS.420.1848D},
\begin{equation}
     f_{c} = \left\{\begin{matrix}1 & T_{tot}< 3\times 10^4\,\mathrm{K} \\
\left ( \frac{T_{tot}}{3\times 10^4\,\mathrm{K}} \right )^{0.82} &3\times 10^4\,\mathrm{K}\leq  T_{tot}\lesssim 10^5\,\mathrm{K} \\
\left ( \frac{72\,\mathrm{keV}}{kT_{tot}} \right )^{1/9}  & T_{tot}\gtrsim 10^5\,\mathrm{K}  \\\end{matrix}\right. ,\label{eq:fc}
\end{equation}
and accounts for scattering effects. %\ob{I think it's more that the total intensity is not affected by the introduction of a color correction factor.  However, you are using an effective temperature for the source of irradiation that only accounts for viscous dissipation.  Perhaps you could iterate to a converged temperature?  I would think it would converge very quickly.}

The angle $\cos\beta$ is the dot product of the normal vector $\vprint{n}$ (eq. \ref{eq:n} or \ref{eq:nbr}, depending on the disk setup) and a unit vector pointing towards the observer. For an observer with viewing angle $\mu$, 
\begin{equation}
    \cos\beta = \vprint{n}\cdot\mathcal{R}_\mu\curlB{0,0,1},\label{eq:cosbeta}
\end{equation}
with $R_\mu$ set by eq.\ref{eq:rot}.

We use eq.\ref{eq:nuFnu} to also test for energy conservation by varying $\cos\beta$ not only in the $\theta$, but also in the $\phi$ direction and integrating over all solid angles. The calculated luminosity integrated over all solid angles deviates from the theoretically expected value (eq.\ref{eq:ldisktheory}) by $<10$\%.
%Note that the observer is always assumed to have a frontal view of the inclined disk region.

% In this section, we calculate the change in the lightcurve variability for our warped and broken disk configuration. We calculate the disk emission using eq. \ref{eq:nuFnu}, assuming that the disks are viewed edge-on but with azimuthal-viewing angles $\mu_s$ varying between 0 and $\pi/2$. Here, $\mu_s=0$ refers to the frontal view of the inclined disk region, and $\mu_s=\pi/2$ to the side view. We calculate the spectra for the precessing disks like in section \ref{subsec:diskspec}, with the same frequency grid and the same $\mu_s$ spacing as for $\mu$. 
% (we discuss the impact of the inclined disk region precessing in section \ref{subsec:timelvary}).%For both the broken and the warped disk setup, $T_{tot}$ depends on both the radius and angle. For warped disks, eq.\ref{eq:cosbeta} will vary with radius and angle as well.  


Only disk portions visible to the observer contribute to eq.\ref{eq:nuFnu}. For $\mu \leq\pi/2$, all warped disk regions are visible. For $\mu>\pi/2$, the innermost region of the warped disk can be shadowed, and an observer may see parts of the top and bottom surface. Extracting the visible regions of the top surface for viewing vectors $R_\mu \curlB{0,0,1}$ and $-R_\mu \curlB{0,0,1}$ gives the total visible surface for $\mu > \pi/2$. A point $P(r,\pi < \phi<2\pi)$ on the top surface of the warped disk is invisible if the angle between its normal vector and the viewing vector is greater than $\pi/2$. To determine whether a point $P_1(r_1,0 < \phi_1<\pi)$ is shadowed by some other point $P_2(r_2,\pi < \phi_2<2\pi)$, we first conduct a binomial search for a 720-entry long angle interval between  $\pi < \phi<2\pi$; for every $\phi$, we minimize the dot product between normal and viewing vector to find the radius $r_{v}$ beyond which the disk is visible to an observer. For a point $P_1(r_1,0 < \phi_1<\pi)$, we then find the corresponding point $P_{v}\anglB{r_{v},\phi_{v}}$ in the observer's line of sight. If the angle between the viewing vector and the horizontal plane is greater than the angle between the horizontal plane and the line $\overline{P_{v}P_1}$, $P_1$ is not visible. To check the visibility of broken disk regions, we collapse the disk onto a two-dimensional plane as seen by the observer. We compare the collapsed positions of the flat region with the collapsed points of the most and least inclined positions, and the collapsed position of the inclined region with the collapsed points of the outermost flat regions to determine whether a point is shadowed. The resulting spectrum is evaluated for a logarithmically spaced 960-entry long frequency grid ranging from $10^{-4}$keV$/h\approx2.4\times10^{13}$ Hz to $20$ keV$/h\approx4.8\times10^{18}$ Hz. The spatial integration is described in section \ref{subsec:numericalEvaluation}.

% An observer will see the inclined region precess over time, resulting in a varying lightcurve. We calculate the spectra during the precession by assuming an edge-on view but with a varying azimuthal-viewing angles $\mu_s$. Here, $\mu_s=0$ refers to the frontal view of the inclined disk region, and $\mu_s=\pi/2$ to the side view. The expression $\cos\beta_s$ due to precession is 
% \begin{equation}
%     \cos\beta_{s} = \vprint{n}\cdot\mathcal{R}_{z,\mu_{s}}\curlB{0,-1,0},\label{eq:cosbetapre}
% \end{equation}
% where $\mathcal{R}_{z,\mu_{s}}$ is a rotation matrix around the z-axis,
% \begin{equation}
%     \mathcal{R}_{z,\mu_{s}}=  \begin{bmatrix}
% \cos\anglB{\mu_{s}} & -\sin\anglB{\mu_{s}} & 0 \\
% \sin\anglB{\mu_{s}} & \cos\anglB{\mu_{s}} & 0 \\
% 0 & 0& 1 \\
% \end{bmatrix}.\label{eq:rotZ}
% \end{equation}

% To calculate the lightcurve variability due to the evolution of $\mu_s$, we note that the total luminosity is not affected by $f_c$ (eq. \ref{eq:fc}). The total luminosity is thus
% \begin{equation}
%     L =\int \frac{\sigma T^4}{\pi}cos \beta_s\,dA.  \label{eq:totLPrecess}
% \end{equation}

% Additionally, we calculate the light curve variability in the 2-12 keV band relevant for RXTE \citep{Jahoda1996SPIE.2808...59J} with eq.\ref{eq:nuFnu}, replacing $\cos\beta$ (eq.\ref{eq:cosbeta}) with $\cos\beta$ (eq.\ref{eq:cosbetapre}). We integrate $L_\nu$ in that energy band with the trapezoidal method, using the integration variable $u=\log{\nu}$ and $du=d\nu/\nu$,
% \begin{equation}
%     L = \int_{2 keV/h}^{12 keV/h} \nu L_\nu\,d\anglB{\log{\nu}}.\label{eq:totL}
% \end{equation}

We calculate spectra for a 20-entry long $\mu$ interval ranging between 0 and $0.95\pi$ of warped and broken disks with $\thmax = 0.1\pi$, 0.2$\pi$, 0.3$\pi$, and $0.4\pi$. To explore the impact of $\rbent$, we also consider warped and broken disks with $\rbent=50r_s$, $500r_s$ and $1000r_s$ with a final inclination of $0.3\pi$ at $\rout$, which requires increasing $\thmax$ to $0.321\pi$ if $\rbent=50r_s$, to $0.38\pi$ if $\rbent=500r_s$, and to $0.44\pi$ if $\rbent=1000r_s$ for the warped disk setup. For another warped disk setup with a final inclination of $0.2\pi$ at $\rout$ and $\rbent=500 r_s$, $\thmax=0.236\pi$. We will state $\rbent$ explicitly for these additional disk configurations. Otherwise, $\rbent=10r_s$. Since $Q_v$, $Q_{irr}$ and thus also the disk spectra depend on $\dot{M}$, we also calculated warped disk spectra with $\rbent=10r_s$, $\thmax=0.3\pi$, and $\dot{M}=0.02\dot{M}_{Edd}$. Unless specified otherwise, $\dot{M}=0.05\dot{M}_{Edd}$, though.

\subsection{Spatial integral evaluation}\label{subsec:numericalEvaluation}

For warped disks, all integrations are evaluated in the unrotated frame. For the broken disk setup, the integrations are performed in the tilted frame, i.e., using $\anglB{r,\tilde{\phi}}$. However, we switch to the unrotated frame when necessary (e.g., for calculating the vectors and $R$ in eq.\ref{eq:dQirr}). %The spatial integration requires in either setup an integration over radius and angle.

The viscous heating rate (eq.\ref{eq:qv}, Fig.\ref{fig:heating}) decreases quickly with radius. Hence, we perform an adaptive integration of eq. \ref{eq:ldisktheory} to split the radial integral into subintegrals with increasing ranges and step sizes. To avoid $Q_v=0$ at $r_\mathrm{isco}$, the first subintegral starts at $\anglB{1+10^{-5}}r_s$ with a radial step size of $\approx3.7\times10^{-5}r_s$, ending at $\approx\anglB{1+4\times10^{-4}}r_s$. The radial step sizes increase up to $625 r_s$ for the last radial integral from $\approx93750r_s$ to $10^5r_s$. 

For the broken disks, the angular integrations in eq. \ref{eq:ldisktheory}, \ref{eq:qint}, and \ref{eq:nuFnu} use a 720-entry long angle interval ranging from 0 to $2\pi$. For the warped disks, eq. \ref{eq:ldisktheory} and \ref{eq:qint} use a 720-entry long angle interval ranging from 0 to $2\pi$ as well, but we exploit the disk symmetry for eq. \ref{eq:nuFnu} with two 192-entry long angle intervals between $0$ and $\pi/2$ and between $3/2\pi$ and $2\pi$ and double the angular integral results to cover all angles; choosing the smaller interval ranges changes the result by less than 1 \%. All integrals are calculated using the Simpson method. 



% The exponential of the blackbody function (eq. \ref{eq:bb}) causes overflow errors for large frequencies and low temperatures. When an overflow occurs, we instead use a Taylor expansion of the exponential,
% \begin{equation}
%     \exp\anglB{x}= \sum_n^N \frac{x^n}{n!},
% \end{equation}
% where $x = h\nu/kT$. We initially set the number of terms $N=100$. In the case the term summation causes an overflow itself, we reduce $N$ until the summation does not raise any errors.

% \begin{figure}
%     \centering
%     \includegraphics[width = 0.8\textwidth]{figures/taylorExp.png}
%     \caption{Caption}
%     \label{fig:taylorExpansion}
% \end{figure}




% \begin{figure}
%     \centering
%     \includegraphics[width = 0.8\textwidth]{newFigures/viewTopspinningDisk.png}
%     \includegraphics[width = 0.8\textwidth]{newFigures/viewEdgespinningDisk.png}
%     \caption{What portions of the disk are visible if the observer sees the disk face-on and edge-on.}
%     \label{fig:visibilityDisk}
% \end{figure}




==> geometryAndIntegral.tex <==
\section{Methods}\label{sec:methods}
\subsection{Disk Geometry}\label{subsec:geometry}
%\ob{Shouldn't the disk only extend down to the ISCO for whatever black hole spin you are assuming?} \jsp{Yes, I agree. I did not really assume a spin when setting up the disk geometries, though. If I wanted the $r_{in} = r_s=r_{isco}$, the corresponding spin paramter should be $a\approx0.9415$, which is somewhat close to the spin parameter used in simulations (the simulations by Liska et al. assume $a=0.9375$). Would it therefore be possible to keep this inner disk radius?}
%The placement of $r_{\mathrm{isco}}$ corresponds to a high black hole spin parameter of $a_*\approx0.95$, making Lense-Thirring precession highly relevant for our disk configurations.
We consider infinitely thin disks extending from the radius of the innermost stable circular orbit $r_{\mathrm{isco}} = r_s$, corresponding to a high black hole spin parameter of $a_*\approx0.95$, to a maximum radius $\rout=10^5r_s$. The radius $r_s$ is the Schwarzschild radius,
\begin{equation}
    r_s = \frac{2GM}{c^2},
\end{equation}
where $G$ is the gravitational constant, $c$ is the speed of light, and $M$ is the black hole mass set to $10M_\odot$. %We assume that the studied disks are infinitely thin (we discuss the impact of the disk thickness in section \ref{sec:discussion}).

In the first considered setup, the accretion disk is warped, and its inclination increases smoothly with radius (section \ref{subsubsec:warpedgeo}). In the second setup, the accretion disk is broken, consisting of a flat inner region and an inclined flat outer disk region (section \ref{subsubsec:brokengeo}). We set both the warp radius, defined as the ratio of the Lense-Thirring precession frequency and the effective kinematic %kinetic
viscosity in the vertical direction \citep{Scheuer1996MNRAS.282..291S}, and the radius separating the flat and inclined region of the broken disk to $\rbent=10r_s$. This choice places the warp and break similarly close to the black holes as in GRMHD simulations \citep[e.g.,][]{Liska2021MNRAS.507..983L,Liska2022ApJS..263...26L}. 

We describe our inclined disks using spherical coordinates $\curlB{r,\theta,\phi}$. %\ob{Normally it is ordered $r$, $\theta$, and $\phi$ to define a right-handed system.}  
Angles in the frame of the disk have a $\sim$ superscript. Angles in the disk and in the unrotated frame are the same in uninclined %flat
disk regions. %In uninclined disk regions, the disk frame is equal to the unrotated frame, so $\Tilde{\phi} = \phi$ and $\Tilde{\theta} = \theta$.

 % For our calculations, we neglect the black hole spin or any impact of magnetic fields.

\subsubsection{Warped Disk Geometry}\label{subsubsec:warpedgeo}
The unit angular momentum vector $\vprint{l} = \curlB{l_x,l_y,l_z}$ of a steady-state, warped accretion disk with constant viscosity is \citep{Scheuer1996MNRAS.282..291S},
\begin{equation} 
\begin{split}
l_x & = \sin\thmax\cos\anglB{2\sqrt{\frac{\rbent}{r}}} \exp\anglB{-2\sqrt{\frac{\rbent}{r}}} \\
 l_y &= \sin\thmax\sin\anglB{2\sqrt{\frac{\rbent}{r}}} \exp\anglB{-2\sqrt{\frac{\rbent}{r}}}\\
l_z &=  \sqrt{1-\anglB{l_x^2 + l_y^2}}.
\end{split}\label{eq:lxlylz}
\end{equation}
leading to a radially dependent disk inclination $i$ of,
\begin{equation}
    i = \cos^{-1}l_z,\label{eq:diskInclination}
\end{equation}
%Keeping only the disk inclination (eq. \ref{eq:diskInclination}) gives 
and disk coordinates in the disk frame
\begin{equation}
\begin{aligned}
    x &=  r\cos\tilde{\phi}\\
    y &= r\sin\tilde{\phi}\cos i\\
    z &= r\sin\tilde{\phi} \sin i.\label{eq:cartesianDisk}
\end{aligned}\end{equation}
Eq.\ref{eq:cartesianDisk} neglects the twisting of the disk implicit in eq.\ref{eq:lxlylz}; the twist is mainly present at small radii (where the inclination
is in any case small) and will thus not majorly impact the implications of the warping at larger radii.
% \begin{equation}
% \begin{aligned}
%     x &= -r\sin\tilde{\phi}\cos i \\
%     y &= r\cos\tilde{\phi}\\
%     z &= r\sin\tilde{\phi} \sin i.\label{eq:cartesianDisk}
% \end{aligned}\end{equation}

Setting eq.\ref{eq:cartesianDisk} equal to the standard definition of spherical coordinates, $\curlB{x,y,z} = \curlB{r\sin\theta\cos\phi, r\sin\theta\sin\phi,r \cos\theta}$, allows solving for $\tilde{\phi}$ in terms of unrotated angles,
\begin{equation}
    \begin{aligned}
    \tilde{\phi} &= \arctan\squB{\frac{\tan\phi}{\cos i}},%\arctan\squB{\tan\tilde{\phi}\cos{i}}
    %\\\theta &= \arccos\squB{\sin\tilde{\phi} \sin i},
\end{aligned}\end{equation}
so that the components of the disk position vector $\vprint{r}=\curlB{x,y,z}$ can be reexpressed as 
% \jsp{should I simplify the expressions further (see commented out version)?}  \ob{Yes, I would, as these expressions are probably computationally better defined and also different from just substituting equation (5) into equation (4).}
\begin{equation}
\begin{aligned}
    x &=  r\cos\anglB{\arctan\squB{\frac{\tan\phi}{\cos i}}} \\
    y &= r\sin\anglB{\arctan\squB{\frac{\tan\phi}{\cos i}}}\cos i \\
    z &= r\sin\anglB{\arctan\squB{\frac{\tan\phi}{\cos i}}} \sin i.\label{eq:carthesianActual}
\end{aligned}\end{equation}

% \begin{equation}
% \begin{aligned}
%     x &=  r\cos\anglB{\arctan\squB{\frac{\tan\phi}{\cos i}}} =\pm r\frac{\cos i}{\sqrt{\cos^2i + \tan^2\phi}}\\
%     y &= r\sin\anglB{\arctan\squB{\frac{\tan\phi}{\cos i}}}\cos i = r\frac{\tan \phi}{\sqrt{\cos^2i + \tan^2\phi}}\cos i\\
%     z &= r\sin\anglB{\arctan\squB{\frac{\tan\phi}{\cos i}}} \sin i=  r\frac{\tan \phi}{\sqrt{\cos^2i + \tan^2\phi}} \sin i.\label{eq:carthesianActual}
% \end{aligned}\end{equation}

\begin{figure}
    \centering
    \includegraphics[width = 0.8\textwidth]{figures/warpedDisk03.png}
    \caption{The inner $r\leq30r_s$ of a warped disk with a maximum inclination of $\thmax=0.3\pi$. The color changes for visualization.}
    \label{fig:warpedDisk}
\end{figure}
Fig. \ref{fig:warpedDisk} shows an example of a warped disk with $\thmax=0.3\pi$. We plot $r\leq30r_s$ and vary the color with radius for visualization. Our parameterization (eq.\ref{eq:carthesianActual}) yields a disk symmetric along the y-axis and antisymmetric along the x-axis.  
% \ob{You need to explain somewhere that you dropped the twist that is inherent in equation (2), and why you did it.}



An area element $dA$ of a warped disk is
\begin{equation}
    dA = \sqrt{\absB{\vprint{v}_r\times \vprint{v}_\phi}}\,dr\,d\phi,\label{eq:dawr}
\end{equation}
where $\vprint{v}_r$ and $\vprint{v}_\phi$ are nonnormalized tangent vectors pointing in the radial and the angular direction respectively, 
\begin{equation}
   \begin{aligned}
    \vprint{v}_r &= \frac{\partial\vprint{r}}{\partial r} \\
    \vprint{v}_\phi &= \frac{\partial\vprint{r}}{\partial \phi} 
    \label{eq:tangentVec}.
\end{aligned}
\end{equation}

The unit normal vector $\vprint{n}$\footnote{The vector $\vprint{n}$ (eq.\ref{eq:n}) approaches $\vprint{l}$ (eq.\ref{eq:lxlylz}) rotated by $\pi/2$ as $r\rightarrow\infty$ and $\phi=\pi/2$. The different pointing direction is due to a different disk orientation and does not impact the results.} is the normalized cross product of $\vprint{v}_r$ and $\vprint{v}_\phi$,
\begin{equation}
    \vprint{n} = \frac{\vprint{v}_r\times \vprint{v}_\phi}{\absB{\vprint{v}_r}\absB{\vprint{v}_\phi}}.\label{eq:n}
\end{equation}
% \ob{Is $\vprint{n}$ the same thing as the unit angular momentum vector $\vprint{l}$ in equation (2), apart from the twist?}

\subsubsection{Broken Disk Geometry}\label{subsubsec:brokengeo}
The broken disk inclination is discontinuous at $\rbent$,
\begin{equation}
     i = \left\{\begin{matrix}
0 & r\leq \rbent \\
\thmax & r > \rbent \\
\end{matrix}\right. .\label{eq:inclBroken}
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width = 0.8\textwidth]{figures/brokenDisk.png}
    \caption{A broken disk setup, where the disk is flat within $r\leq\rbent$ (black region) and inclined by $\thmax=0.3\pi$ otherwise (cyan region). For better visualization, we only plot the region $r\leq30r_s$.}
    \label{fig:brokenDisk}
\end{figure}
The region within $r\leq30r_s$ of a broken disk is shown in Fig. \ref{fig:brokenDisk}. Beyond $\rbent$ (black region), the disk is rotated by $\thmax=0.3\pi$ around the x-axis (cyan region). The rotation by an arbitrary angle $\alpha$ around the x-axis can be described with a rotation matrix $\mathcal{R}_\alpha$,
\begin{equation}
    \mathcal{R}_\alpha=  \begin{bmatrix}
1 & 0 & 0 \\
0 & \cos\anglB{\alpha} & -\sin\anglB{\alpha} \\
0 & \sin\anglB{\alpha} & \cos\anglB{\alpha} \\
\end{bmatrix}.\label{eq:rot}
\end{equation}
For simplicity, we will call the rotation matrix (eq.\ref{eq:rot}) by $\thmax$ $\mathcal{R}$. 
%For the broken disk setup, it is intuitive to first calculate the accretion disk position vector $\vprint{r}$ in the frame of the disk, and then rotate it into the unrotated frame.  In 
The disk coordinates in the unrotated frame therefore are,
\begin{equation}
    \vprint{r} = \left\{\begin{matrix}
r\curlB{\cos\phi,\sin\phi,0} & r\leq \rbent \\
\mathcal{R}\,r\curlB{\cos\tilde{\phi},\sin\tilde{\phi},0} & r > \rbent \\
\end{matrix}\right.,\label{eq:r}
\end{equation}

and the normal vector $\vprint{n}$ is
\begin{equation}
    \vprint{n} = \left\{\begin{matrix}
\curlB{0,0,1} & r\leq \rbent \\
\mathcal{R}\,\curlB{0,0,1} & r > \rbent \\
\end{matrix}\right..\label{eq:nbr}
\end{equation}
The area element $dA$ in the accretion disk frame is 
\begin{equation}
    dA = r\,d\Tilde{\phi}\,dr.\label{eq:dabr}
\end{equation}.




==> introduction.tex <==
\section{Introduction} \label{sec:intro}
% \begin{itemize}
    % \item Accretion disk generally
    % \item tilt of accretion disk: why
    % \begin{itemize}
    %     \item Barden-Peterson effect: flat in - inclined outside \cite{Bardeen1975ApJ...195L..65B,Papaloizou1983MNRAS.202.1181P}
    %     \item evidence of warping: jet - galactic black hole candidate \citep{Hjellming1995Natur.375..464H,Orosz1997ApJ...477..876O}
    %     \item due to supernova (models) \citep{Fragos2010ApJ...719L..79F}
    % \end{itemize}
    % \item why breaking
    % \begin{itemize}
    %     \item physical reason: have torques due to Lense–Thirring precession \citep{Lense1918PhyZ...19..156L} and due to viscosity
    %     \item Lense-Thirring precession has high radial dependence
    %     \item \cite{Nixon2012ApJ...757L..24N}: if $\tau_{LT}>\tau_{\nu}$ breaking
    %     \item observational indications
    % \end{itemize}
    % \item simulations: what happened
    % \item problem with that
% \end{itemize}

% \citep{Nealon2015MNRAS.448.1526N}:break, no mhd
% \cite{Nixon2012ApJ...757L..24N}: break
% Review: \cite{Fragile2024arXiv240410052F}


Accretion disks are ubiquitous in nature, forming around objects ranging from young stars to neutron stars up to supermassive black holes \citep[e.g.,][]{Williams2011ARA&A..49...67W,Alma2015ApJ...808L...3A,EHT2019ApJ...875L...1E,Eijnden2020MNRAS.493.1318V}. For black holes, accretion disks allow the accreted material to move inwards while transporting angular momentum outwards through turbulence (such as that arising from the magnetorotational instability), magnetocentrifugal winds, and possibly spiral waves
\citep[e.g.,][]{Blandford1982MNRAS.199..883B,Balbus1998RvMP...70....1B,Spruit1989ASIC..290..325S,MunozDarias2019ApJ...879L...4M}. %The accretion disk structure depends on the mass accretion rate. If the mass accretion rate is high, accretion disks are expected to be geometrically thin but optically thick.
% The black hole spin affects accretion disks as well, impacting properties such as the radius of innermost stable circular orbit \citep[e.g.,][for a review on black hole accretion, see \cite{Abramowicz2013LRR....16....1A}]{Bardeen1972ApJ...178..347B}.

%. Supermassive black holes might have grown through the accretion of gas with randomly oriented angular momentum vectors
The angular momentum vector of the accreted material can misalign with the black hole spin axis. The misalignment can arise for instance through natal kicks during supernovae \citep[e.g.,][]{Kalogera2000ApJ...541..319K,Gerosa2013PhRvD..87j4028G}, or due to turbulent accretion during galaxy mergers \citep[][]{King2006MNRAS.373L..90K}. Observationally, misalignment of accretion disks has been indicated by precessing jets and from gravitational wave measurements   
%The possibility of a misalignment between the angular momentum of the accretion flow and the black hole spin axis is supported by observations of gravitational waves and jet orientations 
\citep[e.g.,][]{Hjellming1995Natur.375..464H,Orosz1997ApJ...477..876O,OShaughnessy2017PhRvL.119a1101O,Cui2023Natur.621..711C}.%appear to support the idea of black hole spin axis being misaligned with the angular momentum axis of the accretion flow or the binary system %showed that accretion of gas with randomly orientated angular momentum vectors is a possible pathway to form the supermassive black holes observed at high redshifts \citep[e.g.,][]{Barth2003ApJ...594L..95B}.
% \ob{WE HAVE TO BE CAREFUL WHEN REFERRING TO SUPERMASSIVE BLACK HOLES AND AGN, AS THEY DON'T REALLY HAVE A SOFT STATE WHICH MATCHES REALLY WELL WITH MULTICOLOR BLACKBODIES.  IT IS OKAY HERE, BUT WE HAVE TO BE CAREFUL LATER WHEN DISCUSSING WHAT HAS BEEN CONSTRAINED.}


%\cite{Bardeen1975ApJ...195L..65B} coined the 'Bardeen-Peterson' effect; %in their calculations, later improved by \cite{Papaloizou1983MNRAS.202.1181P}, 
%a thin disk aligns with the black hole spin axis close to the black hole, and transitions to an inclined disk at larger radii. %smoothly changes in the calculations by \cite{Bardeen1975ApJ...195L..65B}, the disk inclination can also lead to discontinuities.  The first simulations testing the impact of Lense-Thirring precession relied on smoothed particle hydrodynamics, and found the disks to tear 
The misalignment of the black hole spin axis and the angular momentum axis of the accretion flow will impact the accretion flow structure \citep[for a review on tilted accretion disks, see, e.g.,][]{Fragile2024arXiv240410052F}. An inclined disk around a spinning black hole experiences Lense-Thirring precession, which induces torque on the disk. In the calculations by \cite{Bardeen1975ApJ...195L..65B}, Lense-Thirring precession aligns the accretion disk with the black hole spin at small radii, and the disk smoothly transitions into an inclined disk at larger radii. However, the torque due to Lense-Thirring precession increases with inclination angle, and the disk can fracture when it surpasses viscous torques \citep{Nixon2012ApJ...757L..24N}. Smoothed particle hydrodynamics simulations found disk tearing to occur for inclinations $\gtrsim45^\circ$ \citep[e.g.,][]{Nelson2000MNRAS.315..570N,Nixon2012ApJ...757L..24N,Nealon2015MNRAS.448.1526N}. Disks breaking at inclinations $\gtrsim45^\circ$ have also been found in GRMHD simulations, with the difference that the disk warp or break occurs closer to the black hole \citep[e.g.,][]{Liska2019MNRAS.487..550L,Liska2021MNRAS.507..983L,Liska2022ApJS..263...26L}. %In contrast to earlier work though, GRMHD simulations place %. However, disagreements about the inclined disk structure remain; GRMHD simulations place the location of the break or warp closer to the black hole than predicted in earlier analytical work and simulations.

% The dependence of the disk continuity on the inclination angle has been repeatedly demonstrated in both smoothed particle hydrodynamic simulations as well as GRMHD simulations \citep[e.g.,][]{Nixon2012ApJ...757L..24N,Nealon2015MNRAS.448.1526N,Liska2019MNRAS.487..550L,Liska2021MNRAS.507..983L,Liska2022ApJS..263...26L}. %ran smoothed particle hydrodynamic simulations, and found slightly inclined disks to be continuous but highly inclined disks to break apart. Similarly, \cite{Liska2019MNRAS.487..550L} and \cite{Liska2021MNRAS.507..983L} ran GRMHD simulations of thin tilted accretion disks. For slightly tilted disks with an inclination of 10$^\circ$, the simulated disks by \cite{Liska2019MNRAS.487..550L} smoothly transitioned from flat to being inclined, but inclinations of $\geq45^\circ$ caused disk breaking \citep{Liska2021MNRAS.507..983L,Liska2022ApJS..263...26L}. 

Given the significant impact of Lense-Thirring precession on the accretion disk structure in simulations, the question arises as to how the inclined accretion disk structure translates into observational properties. %If warped and broken disks occur frequently in nature, their disk structure should not noticeably affect their emission.  \ob{I commented this out in order for the paragraph to flow better.}
The soft state of a stellar-mass black hole is dominated by thermal emission, which is thought to originate from a geometrically thin but optically thick accretion disk \citep[e.g.,][]{Dotani1997ApJ...485L..87D,Frontera2001ApJ...546.1027F}. If the disk is misaligned with the black hole spin axis, this emission should come from a warped or broken disk. Nevertheless, black hole systems with high orbital inclinations and spins can be adequately modeled as a multitemperature, color-corrected %multicolor
blackbody, with the blackbody temperature varying with radius \citep[e.g.,][]{Makishima1986ApJ...308..635M}, emitted by a flat disk \citep[e.g.,][]{Gierlinski2004MNRAS.347..885G,Mall2024MNRAS.52712053M}. %\jsp{\cite{Mall2024MNRAS.52712053M} fit the disk inclination. However, this inclination agrees with the orbital inclination \citep{YanezRizo2022MNRAS.517.1476Y}.}
%besides the impact of general relativistic effects and atomic processes, a model of a multicolor blackbody, with the blackbody temperature varying with radius \citep[e.g.,][]{Makishima1986ApJ...308..635M}, coming from a flat disk can provide an adequate fit to the observed thermal emission around black holes with high inferred spins \citep[e.g.,][]{Gierlinski2004MNRAS.347..885G,Mall2024MNRAS.52712053M}. %{Davis2006ApJ...647..525D,Mudambi2020MNRAS.498.4404M,Aneesha2024MNRAS.tmp.1757A}
%Since flat disk models can represent the observed emission well, 
If the disks around these black hole systems are warped or broken, their emission should therefore resemble the emission of an inclined flat disk. %\ob{We will need to be more precise here.  Some of the best constraints come from LMC X-3, but this has a low-spin black hole so it is not clear that it is relevant.  There are other BHXRBs that we can cite, though.}  
In this work, we test the inclined disk geometry of GRMHD simulations and compute the emission of warped and broken disks around stellar-mass black holes and compare them with flat-disk multicolor blackbody spectra. For this comparison, the paper is structured as follows. The calculations of the disk emission are described in section \ref{sec:methods} and presented in section \ref{sec:results}. We discuss our results in section \ref{sec:discussion} and conclude with section \ref{sec:conclusion}.
%It has been suggested that disk breaking could be a possible origin of often observed quasi-periodic oscillations \citep{Musoke2023MNRAS.518.1656M}.

%the smoothness of the transition between the flat and the tilted disk portion has been called into question in simulations.

==> results.tex <==
\section{Results}\label{sec:results}
\subsection{Disk Spectra}\label{subsec:discspectra}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/spectraBoth.png}
%     \caption{...}
%     \label{fig:bothSpectra}
% \end{figure}

% Fig. \ref{fig:bothSpectra} shows spectra of the warped disk (left panel) and the broken disk (right panel), viewed face on (black solid lines) and at an angle of $0.4\pi$ (blue dash-dotted lines). For both setups, $\thmax=0.4\pi$. Each panel also features the spectra of a flat disk viewed face on (gray dotted lines) and at an angle of $0.4\pi$ (cyan dashed lines) for comparison. The warped disk spectra vary negligibly from the flat disk ones.


% \subsection{Warped disks}\label{subsec:warpedResults}
% \begin{itemize}
%     \item spectra
%     \item power law at low energies
% \end{itemize}

\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/spectraWarped3New.png}
    \caption{Spectra of the warped disk with $\thmax=0.3\pi$ (black solid lines) and flat disk (blue dashed lines) when viewed at an angle of $\mu=0$ (a), $\mu = 0.2\pi$ (b), and $\mu=0.4\pi$ (c), and $\mu=0.6\pi$ (d). The warped-disk emission at low energies is enhanced due to self-irradiation and a projected area increasing the closer $\mu$ is to $\pi/2$.}
    \label{fig:spectraWarped}
\end{figure*}

Fig. \ref{fig:spectraWarped} shows spectra of a warped disk with $\thmax=0.3\pi$ (black solid lines) and a flat disk (blue dashed lines), viewed face on (a), and at angles $0.2\pi$ (b), $0.4\pi$ (c), and $0.6\pi$ (d). The plotted high-energy emission of the flat and the warped disk agree with each other in panels a-c, because it predominantly originates from the flat inner region where the effects of self-irradiation are unimportant (Fig. \ref{fig:heating}, left panel). If $\mu = 0.6\pi$ (d), the innermost region is not visible and only the outer cooler regions contribute to the observed emission, shifting the spectrum to low energies. The low-energy emission of the warped disk dominates over the flat disk emission for all $\mu$ due to self-irradiation increasing the temperatures at large radii (Fig. \ref{fig:heating}), and because the projected area of the outer warped region increases the closer $\mu$ is to $\pi/2$. %Hence, the emission originating from the outer warped region contributes more significantly with increasing $\mu$, and the $Q_{irr}>Q_v$ in this region causes the spectra to increasingly deviate from flat disk spectra.



\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/spectraBroken3new.png}
    \caption{Same as Fig.\ref{fig:spectraWarped}, but for a broken disk with $\thmax=0.3\pi$. The large inclination of the majority of the broken disk region leads to palpable differences between the broken (black solid lines) and flat spectra (blue dotted lines).}
    \label{fig:spectraBroken}
\end{figure*}
Fig. \ref{fig:spectraBroken} shows spectra of a broken disk for the same viewing angles and $\thmax$ as in Fig. \ref{fig:spectraWarped}. Like for the warped disk, the high-energy emission of the broken and flat disk agree with each other. The low energy emission comes largely from the outer inclined region. In contrast to warped disks, the low-energy emission is not significantly enhanced through self-irradiation because $Q_v$ always dominates over $Q_{irr}$ (Fig. \ref{fig:heating}). The low-energy emission $\leq1$ keV of the flat disk is $\approx1.46$ times greater than of the broken disk when $\mu=0$ (a) due to the outer disk being inclined by $\thmax$. In panels b-d, the broken disk emission dominates at low energies because the effective viewing angle of the inclined outer disk is smaller than for the flat disk.

%At $\mu=0$ (a), the observer sees the outer region inclined by $\thmax$, causing the $\mu=0$ broken disk spectrum to have a $\approx1.2$ times smaller amplitude than the flat disk one. The broken and flat disk spectra at $\mu=0.2\pi$ are nearly identical, because the effective viewing angle of the inner and inclined region is the same as for the flat disk. When $\mu=0.4\pi$, the observer effectively sees the inclined region face-on, resulting in a $\approx1.3$ times greater amplitude of the broken disk spectrum compared to the flat disk one.

%\ob{I really worry that many (but not all) of the figures you show have the broken or warped disk spectrum exceeding that of the flat disk - a competent referee will likely demand that you demonstrate global energy conservation, so that the total luminosity of the disk over all frequencies and viewing angles is the same no matter what the disk geometry.}

% While the broken disk configuration may yield a spectrum similar to a flat disk at first glance, their power-law indices differ from the multicolor blackbody solution. 
Self-irradiation and the projected area of the outer disk region introduces significant differences in the power-law indices at low energies compared to the multicolor blackbody solution (Fig. \ref{fig:expboth}). A multicolor blackbody scales at low energies as $\nu L_\nu\propto\nu^{\gamma}$ with a power-law index of $\gamma=4/3$ \citep[black solid line, e.g.,][]{Makishima1986ApJ...308..635M}. The unfilled circle marks the absence of a multicolor blackbody power-law index at $\mu=\pi/2$, because no emission is observed from an edge-on infintely flat disk. Fitting a power-law to the multicolor blackbodies plotted in Fig. \ref{fig:spectraWarped} and \ref{fig:spectraBroken} in the 0.2-0.5 keV range yields $\gamma\approx1.36$ for all viewing angles, deviating from $\gamma=4/3$ by $\leq2\%$. The power-law indices for that energy range of the warped disk vary between $\gamma\approx0.91-1.26$ at $\mu=0$, with $\gamma$ decreasing with $\thmax$ (left panel). As the inner disk region becomes less visible and the outer disk region more visible, $\gamma$ decreases with increasing $\mu$. The indices become negative when the inner region is completely shadowed and the visible emission peaks at energies $\lesssim0.2$ keV (see rightmost panel in Fig. \ref{fig:spectraWarped}). As $\mu$ increases further, the innermost region is visible again, and $\gamma$ sharply increases before slightly decreasing again.

The power-law indices of broken disks fitted between 0.2 and 0.5 keV decrease for $\mu\leq\pi/2$ in a similar fashion %likewise
(Fig. \ref{fig:expboth}, right panel). Starting with $\gamma\approx1.37-1.54$ at $\mu=0$, the decrease is approximately linear; combining the linear fits for this $\mu$ range gives $\gamma(\theta,\mu \leq \pi/2) = \anglB{a\,\thmax+b}\mu + \anglB{c\,\thmax+d}$, where $a = -0.10\pm0.02$, $b=-0.09\pm0.01$, $c = 0.10\pm0.03$, and $d=1.36\pm0.02$. The inclined region is viewed edge-on at $\mu=\pi/2+\thmax$, raising $\gamma$ to a maximum value of $\approx2.66$ regardless of $\thmax$. The multicolor blackbody solution $\gamma=4/3$ holds in the energy range $kT_{out}\ll E\lesssim0.3k T_{in}$, where $T_{in}$ and $T_{out}$ are the inner and outer disk temperatures respectively \citep{Makishima1986ApJ...308..635M}. Since the visible flat portion only extends out to $\rbent$, the temperatures do not vary enough for that energy range to be applicable. Hence, $\gamma$ significantly differs from the multicolor blackbody solution even when only the flat disk portion is visible.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/exponent.png}
    \caption{Left panel: The power-law indices of $\nu L_\nu$ between 0.2 keV and 0.5 keV for warped disks for different viewing angles. The indices decrease with decreasing visibility of the innermost disk region and increase again with its regained visibility. Right panel: Same as the left panel, but for broken disks. The indices decrease with increasing $\mu\leq\pi/2$. The sudden increase in $\gamma$ is due to the inclined region being viewed edge-on. The power law indices of the inclined disks significantly differ from the multicolor blackbody solution (black solid lines).}
    \label{fig:expboth}
\end{figure}


The deviations between inclined and flat disks decrease with increasing $\rbent$. Fig.\ref{fig:spectraChangeRW} shows spectra (eq.\ref{eq:nuFnu}) of warped disks (left panel) and broken disks (right panel) with a maximum inclination of $\approx0.3\pi$ at $\rout$ for $\mu=0.4\pi$ and $\rbent=10r_s$ (black solid lines, same as in panel c of Fig. \ref{fig:spectraWarped} and \ref{fig:spectraBroken} respectively), $\rbent=50r_s$ (purple dotted lines), $\rbent=500r_s$ (orange dot-dashed lines), and $\rbent=1000r_s$ (grey dash-dotdotted lines). Increasing $\rbent$ reduces the projected area of the outer disk regions and confines $Q_{irr}>Q_v$ for warped disks to increasingly larger radii. Hence, the differences at low energies between the inclined and the flat disk spectra (blue dashed lines) decrease. 

The reduction of the low-energy emission is reflected in $\gamma$ fitted between 0.2 keV and 0.5 keV. The power-law indices of the warped disk with $\rbent=10r_s$ (blue dashed line in the left panel of Fig. \ref{fig:expboth}) are significantly lower than the multicolor blackbody solution $\gamma=4/3$ for the majoritiy of viewing angles. While moving $\rbent$ to $50r_s$ and adjusting $\thmax$ to $0.321\pi$ reduces the low-energy emission $\gtrsim0.2$ keV, $\gamma$ does not significantly converge towards the flat disk solution for the calculated viewing angles; $\gamma$ still deviates by $\gtrsim15$\% for the warped disk. Increasing $\rbent$ further to $500r_s$ and $1000r_s$ and increasing $\thmax$ to $0.38\pi$ and $0.44\pi$ respectively moves $\gamma$ towards $4/3$. Except for $\mu=1/2\pi-3/4\pi$, when the innermost region of the warped disk is not visible, $\gamma$ deviates from $4/3$ by $\lesssim31$ \% if $\rbent=500r_s$ and by $\lesssim6$\% if $\rbent=1000r_s$ and the disk is warped. 

The power-law indices for the 0.2 keV - 0.5 keV range converges towards $4/3$ with increasing $\rbent$ for broken disks likewise. The broken disk with $\thmax=0.3\pi$ had $\gamma$ varying between $\approx1.15$ ($\approx1.19$ when ignoring $\mu=\pi/2$) and $\approx2.66$ (blue dashed line in the right panel of Fig. \ref{fig:expboth}). Increasing $\rbent$ reduces the peak in $\gamma$ at $\mu=\pi/2+\thmax$, because the energy range $kT_{out}\ll E\lesssim0.3k T_{in}$ is increasingly satisfied by the flat disk region. In addition, $\gamma$ decreases at $\mu=\pi/2$, because an increasingly smaller area is visible. Increasing $\rbent$ to $50 r_s$ and ignoring $\mu=\pi/2$ changes the $\gamma$ range to $\approx0.62-2.18$. Raising $\rbent$ further to $500 r_s$ and $1000 r_s$ makes $\gamma$ increasingly indistinguishable from the multicolor blackbody solution; ignoring $\mu=\pi/2$, $\gamma$ varies between $\approx1.12-1.37$ and $\approx1.34-1.36$ respectively.

Discerning flat and inclined disks through observations will depend on the disk inclination and the observed energy band. A warped disk with $\thmax=0.236\pi$ and $\rbent=500 r_s$ has power-law indices deviating by $\lesssim15$\% from $\gamma=4/3$ for $\mu$ excluding $\pi/2-0.65\pi$, when the innermost region is not visible, and is thus more similar than a warped disk with $\thmax=0.38$ and $\rbent=500 r_s$. The differences between flat and inclined disks are also reduced when contentrating only on the high-energy emission (see Fig. \ref{fig:spectraWarped}, \ref{fig:spectraBroken}). For example, while $\gamma$ of the broken disk with $\thmax=0.3 \pi$ and $\rbent=10r_s$ deviates by a factor of $\approx2$ from $\gamma=4/3$ if $\mu=0.8\pi$, its emission at 8 keV deviates from the flat disk emission only by a factor of $\approx1.16$ for that viewing angle. However, being able to recoup the characteristic power-law index  $\gamma=4/3$ of a multicolor blackbody emission necessitates $\rbent\geq50r_s$.
% \ob{I worry a bit about gamma=4/3 being the standard of comparison.  It's interesting that your solutions converge to this if the warp or break radius is large enough, but I would also have expected it to be flatter simply because in that X-ray energy range you are approaching the peak of the multitemperature disk spectrum.  If we lowered the accretion rate below 0.5 Eddington, that peak would shift to lower energies.  It might all be okay, but could it be that the irradiation is less of an issue for lower Eddington ratios?}
% \jsp{I still need to finish this paragraph.}
% the amplitude of the inclined disk spectra. While disk heating is still important for all warped disk setups (left panel), their spectra deviate from the multicolor emission (blue dashed lines) at increasingly lower energies. For $\mu=0.4$, the warped disk with $\rbent=10r_s$ (black solid line, same as in the right panel of Fig. \ref{fig:spectraWarped}) deviates from the multicolor blackbody emission by more than 10\% at $\lesssim 5.1$ keV, the $\rbent=50r_s$ disk (orange dotted line) at energies $\lesssim 1.2$ keV, and the $\rbent=200r_s$ disk (orange dotted line) at energies $\lesssim 0.5$ keV.

% The broken disk (right) panel shows significant deviations from the multicolor blackbody emission (blue dashed line) for $\rbent=10r_s$ (black solid line), and $\rbent=50r_s$ (orange dotted line) as well, with deviations by more than 10\% at $\lesssim 3.4$ keV and $\lesssim 1.1$ keV respectively if $\mu=0.4\pi$. In contrast, increasing $\rbent$ to $200r_s$ moves deviations from the multicolor blackbody emission by more than 10\% to $\lesssim 0.4$ keV. \jsp{I should probably add another sentence about the takeaway message here.}  \ob{Something along the lines of how far out $r_\mathrm{f}$ would have to be to make deviations less than ten percent in some energy range.  Again, quantitative information will be of most use to observers.}

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/spectraChangeRW_warp.png}
    \caption{Spectra of warped (left panel) and broken (right panel) disks for $\rbent=10r_s$ (black solid lines, same as in panels c of Fig. \ref{fig:spectraWarped} and \ref{fig:spectraBroken} respectively), $\rbent=50r_s$ (purple dotted lines), $\rbent=500r_s$ (orange dot-dashed lines), and $\rbent=1000r_s$ (grey dash-dotdotted lines) for $\mu=0.4$. The inclination at $\rout$ is $\approx0.3\pi$ for all disks. Increasing $\rbent$ reduces the differences between inclined and flat disk (blue dashed lines) spectra.}
    \label{fig:spectraChangeRW}
\end{figure}







% Fitting a power-law to the flat disk emission between 0.2 keV and 0.5 keV, we find $\gamma\approx1.36$ for all viewing angles except when $\mu=0.5\pi$, because no emission is observed when an infinitely thin disk is viewed edge on. Since the broken disk spectra is similar to a superposition of two multicolor blackbody emissions, coming from the flat disk and the inclined disk region, $\gamma$ varies with viewing angle and $\thmax$. For $\thmax=0.4\pi$ and $\mu=0$ for instance (left panel in Fig. \ref{fig:spectraBroken}), fitting a power-law between 0.1 keV and 0.5 keV yields $\gamma\approx1.54$. If $\mu=0.2$, however, the $\thmax=0.4\pi$ will have the same low-energy power-law coefficent of $\gamma\approx1.37$ as a multicolor blackbody (middle panel in Fig. \ref{fig:spectraBroken}). Thus, except when the effective viewing angle of the inclined region is the same as of the flat disk region, a broken disk emission differs from a multicolor blackbody at low energies.


% \jsp{I could add a figure of $\gamma$ vs $\mu$, but this might not be necessary.}  \ob{Actually, I think that would be a really great idea, as it would be very useful for observers.}

% The spectral differences between inclined and flat disks (Fig. \ref{fig:spectraWarped}, \ref{fig:spectraBroken}) can be captured with a spectral power-law index $\gamma$ at low energies (Fig. \ref{fig:expboth}). To calculate the spectral power-law index, we fit a power-law to the emission between 0.1 keV and 0.5 keV.  We find that $\gamma\approx1.37$ for the flat disk regardless of the viewing angle (black solid lines in Fig. \ref{fig:expboth}) and therefore reasonably close to the theoretically expected value. 

% As visible in Fig. \ref{fig:spectraWarped}, the emission of a warped disk has a shallower gradient at low energies, leading to a smaller power-law index regardless of $\thmax$ and $\mu$ than the flat disk $\gamma$ (left panel). Due to the greater warp, $\gamma$ is smaller for greater $\thmax$. With the emission from the outer regions powered increasingly by $Q_irr$ (Fig.\ref{fig:heating}, left panel) dominating the spectrum at large $\mu$, $\gamma$ decreases with viewing angle.

%The power-law index of the broken disks decreases with viewing angle as well (right panel). If the disks are seen face-on, though, $\gamma$ is greater for the broken than for the flat disk, and the difference increases with $\thmax$. For $\thmax=0.4\pi$, $\gamma\approx1.54$ at $\mu=0$. As already seen in Fig. \ref{fig:spectraBroken}, the contribution of the inclined disk region increases with $\mu$, which decreases $\gamma$. The power-law index decrease is the strongest for the $\thmax=0.4\pi$ broken disk, which has $\gamma\approx1.20$ at $\mu=0.49\pi$. But also less inclined broken disks have a significant reduction in $\gamma$ at higher viewing angles. At $\mu=0.49\pi$, $\gamma$ of all broken disk setups differ by more than 10\% of the theoretically anticipated value of a multicolor blackbody.

%and is scaled differently with viewing angle than for the flat disk. When viewed face on, the  and the scaling with the disk inclination can either reduce (left panel) or enhance (middle and right panel) its emission compared to the flat disk contribution, depending on $\thmax$ and $\mu$.   


% If viewed face-on (left panel), the flat disk (blue dashed lines) and broken disk emission (black solid lines) is comparable at energies $\gtrsim 6$ keV. However, the broken disk emission at lower energies is reduced compared to the flat disk one 


%The disk beyond $\rbent$ radiates at lower energies than the region within $\rbent$ because of the temperatures decreasing with radius. Since the inclined region is less aligned with the viewing direction than the flat disk, the spectral contribution of the inclined region is reduced, and the amlplitude of the face-on spectrum of the flat disk is $\approx1.18$ times greater than for the broken disk. However, with increasing $\mu$ the inclined disk is increasingly more aligned with the viewing direction. While the amplitude of the broken spectrum decreases for $\mu=0.3\pi$ (center panel) and $\mu=0.49\pi$ (right panel), the tilted disk portion causes the broken emission to surpass the flat one. When the two disks are viewed with $\mu=0.49\pi$ nearly edge-on, the broken spectra amplitude is $\approx8.62$ times greater than the flat one.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/exponent.png}
%     \caption{The power-law index of $\nu L_\nu$ between 0.1 keV and 0.5 keV for different viewing angles for the warped disk (left panel) and broken disk (right panel) setup. The power law indices of the inclined disks differ from the flat disk value (black solid lines) and decrease with increasing viewing angle.}
%     \label{fig:expboth}
% \end{figure}


% \subsection{Time-variability}\label{subsec:timelvary}
% % The luminosity of an inclined accretion disk will vary as the inclined disk region precesses. 

% % Since the RXTE telescope \citep{Jahoda1996SPIE.2808...59J} conducted many of the black hole observations \citep[e.g.,][]{Belloni2005A&A...440..207B,Motta2011MNRAS.418.2292M}, we integrate $L_\nu$ between 2-12 keV with the trapezoidal method to calculate the light curve variability. 
% % \textcolor{red}{It might make sense to integrate only within an energy band relevant for observations. I could use the RXTE band, for example, and integrate $L_\nu$ between 2-12 keV.}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/L_precess.png}
%     \caption{The total luminosity (eq.\ref{eq:totL}) for warped (left panel) and broken disks (right panel) as the inclined region precesses. The precession of the inclined region from the front to the side view reduces the total luminosity by over an order of magnitude for warped disks and down to zero for broken disks. }
%     \label{fig:L_precess}
% \end{figure}
% Fig.\ref{fig:L_precess} shows the integrated luminosity (eq.\ref{eq:totLPrecess}) as $\mu_s$ varies from 0  (frontal view) to $0.5\pi$ (side view) for warped (left panel) and broken disks (right panel). With the precession of the warp, the luminosity of the warped disk varies by over an order of magnitude regardless of $\thmax$ (left panel). An infinitely thin broken disk has no projected area when viewed from the side, so the integrated luminosity becomes zero at $\mu_s=0.5\pi$ for all $\thmax$ (right panel). While physical disks are not infinitely thin (see also section \ref{sec:discussion}) and could have some warping or twisting in its inner region \citep[e.g.,][]{Liska2022ApJS..263...26L}, a broken disk should experience a significant drop in luminosity with the precession of the inclination nevertheless. 

% The luminosity variability depends on the considered energy band. Since the outer inclined disk region visible in the edge-on view primarly emits at low energies, considering only the RXTE \citep{Jahoda1996SPIE.2808...59J} energy band of 2-12 keV limits the variability to a factor of $\approx7.4$ for the warped disks (eq. \ref{eq:totL}). Due to the assumed infinite thinness of the broken disks, their luminosity would still decrease to 0 at $\mu_s=0.5\pi$. A broken disk with some vertical extent would have a lower variability in the 2-12 keV band compared to considering all energies, but a considerable luminosity variation can still be expected.  \ob{There is an additional caveat - even broken disks will likely have some twist, implying that there is no viewing angle where the disk will be perfectly edge-on everywhere.  This caveat should be acknowledged.}\jsp{I mentioned it in the paragraph before this one.}

% Despite restricting the energy band, the calculated luminosity variability disagrees with observations. The precession of the inclined disk region should lead to periodic variations in the lightcurve. However, the soft state of black hole systems displays little variability with a fractional root mean square variability of $<3\%$\citep[for a review, see][]{Kalemci2022hxga.book....9K}. While weak quasi-periodic oscillations have been observed during the soft state, they are rare and appear to be driven by the comptonizing region and not by the accretion disk \citep[e.g.,][]{Casella2005ApJ...629..403C,Zhang2023MNRAS.526.3944Z}. The little variability of the accretion disk emission suggest that the precession of the inclined disk region should not impact the lightcurve significantly, which could be achieved with limiting the inclined region to larger radii (see also section \ref{sec:discussion}).%Even highly spinning black hole systems with a potentially warped accretion disk such as Cygnus X-1 feature stable disk emission features; \cite{Walton2016ApJ...826...87W} observed Cygnus X-1 with NuSTAR, and found disk reflection features such as the inferred black hole spin to be constant accross different observations, suggesting a      %\jsp{I should propably add on what timescale the lightcurves of our disks should vary. If the disk is not viewed edge-on, a precession would probably not cause such a great variation in the lightcurve. I could refer to some distribution of viewing angles for black hole systems.}  \ob{Also, you should try and be more quantitative about the observations.  What are some upper limits on variability on the soft-state?}

% While more complex tilted accretion disk structures may introduce additional deviations from a flat multicolor spectrum as outlined above, the deviations decrease with the inclination starting at larger radii. Moving $\rbent$ outward reduces $Q_{irr}$ (eq.\ref{eq:qint}) and the projected area of the inclined disk region. 


% We test the impact of moving $\rbent$ out to $50r_s$ and $200 r_s$ for a warped and broken disk configuration. We aim for an angle of $0.3\pi$ at the outermost radii (eq.\ref{eq:diskInclination}), so we increase $\thmax$ to $0.321\pi$ for $\rbent=50r_s$ and to $0.345\pi$ for $\rbent=200r_s$ if the disk is warped.
